First measurement of Gallium Arsenide as a low-temperature calorimeter

In this paper, we present the first measurement of a Gallium Arsenide crystal working as low-temperature calorimeter for direct Dark Matter (DM) searches within the DAREDEVIL (DARk-mattEr DEVIces for Low energy detection) project. In the quest for direct dark matter detection, innovative approaches to lower the detection thershold and explore the sub-GeV mass DM range, have gained high relevance in the last decade. This study presents the pioneering use of Gallium Arsenide (GaAs) as a low-temperature calorimeter for probing the dark matter-electron interaction channel. Our experimental setup features a GaAs crystal at ultralow temperature of 15 mK, coupled with a Neutron Transmutation Doped (NTD) thermal sensor for precise energy estimation. This configuration is the first step towards the detection of single electrons scattered by dark matter particles within the GaAs crystal, to significantly improve the sensitivity to low-mass dark matter candidates.

==> Makefile <==
# input
MAIN					= main

MAIN_TEX				= ${MAIN}.tex
MAIN_PDF				= ${MAIN}.pdf

BIBLIOGRAPHY		= ref.bib

# clean
FILE_CLEAN			= *.aux *.bbl *.blg *.brf *.idx *.ilg *.ind *.log *.out *~ *Notes.bib
FILE_DISTCLEAN		= ${MAIN_PDF} ${OUTPUT_PDF}

.PHONY:	pdf biblio \
			rename \
			distclean clean

pdf:	${MAIN_TEX}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
biblio: ${MAIN_TEX} ${BIBLIOGRAPHY} 
	pdflatex ${MAIN}
	bibtex ${MAIN}
#	makeindex ${MAIN}
	pdflatex ${MAIN}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
view:	${MAIN_PDF}
	evince ${MAIN_PDF}
	
distclean:	clean
	rm -f ${FILE_DISTCLEAN}

clean:
	rm -f ${FILE_CLEAN}

